A Matrix Chernoff Bound for Markov Chains and Its Application to Co-occurrence Matrices

We prove a Chernoff-type bound for sums of matrix-valued random variables sampled via a regular (aperiodic and irreducible) finite Markov chain. Specially, consider a random walk on a regular Markov chain and a Hermitian matrix-valued function on its state space. Our result gives exponentially decreasing bounds on the tail distributions of the extreme eigenvalues of the sample mean matrix. Our proof is based on the matrix expander (regular undirected graph) Chernoff bound [Garg et al. STOC '18] and scalar Chernoff-Hoeffding bounds for Markov chains [Chung et al. STACS '12]. Our matrix Chernoff bound for Markov chains can be applied to analyze the behavior of co-occurrence statistics for sequential data, which have been common and important data signals in machine learning. We show that given a regular Markov chain with $n$ states and mixing time $\tau$, we need a trajectory of length $O(\tau (\log{(n)}+\log{(\tau)})/\epsilon^2)$ to achieve an estimator of the co-occurrence matrix with error bound $\epsilon$. We conduct several experiments and the experimental results are consistent with the exponentially fast convergence rate from theoretical analysis. Our result gives the first bound on the convergence rate of the co-occurrence matrix and the first sample complexity analysis in graph representation learning.

==> deepwalk.tex <==
\section{DeepWalk}

DeepWalk~\cite{perozzi2014deepwalk}

\begin{algorithm}[h]
\caption{DeepWalk (a matrix factorization view)}
\label{alg:dw}
\For{$n = 1,2,\ldots, N$}{
Sample a vertex $v^n_1$ from a distribution\;
Generate a vertex sequence $(v^n_1, \cdots, v^n_L)$ of length $L$ by a random walk on graph $G$\;
\For{$j = 1,2,\ldots, L-T$}{
\For{$r = 1, \ldots, T$} {
	Add vertex-context pair $(v^n_j, v^n_{j+r})$ to multiset $\mathcal{D}$\;
    Add vertex-context pair $(v^n_{j+r}, v^n_j)$ to multiset $\mathcal{D}$\;
}}}
%Run SGNS on $\mathcal{D}$ with $b$ negative samples.
Factorize a matrix with its entry at $w$-th row and $c$-th column to be $\log{\left(\frac{\#(w, c) \abs{\mathcal{D} }}{b\#(w) \cdot \#(c)}\right)}$.
\end{algorithm}


From \cite{qiu2018network}, we already knew that

\begin{theorem} When $L\rightarrow\infty$, we have
    \label{thm:fraction}
    \beq{
    \nonumber
    \frac{\#(w, c)}{\abs{\mathcal{D} }} \overset{p}{\to} \frac{1}{2T} \sum_{r=1}^T \left( \frac{d_w}{\vol(G)}\left(\bm{P}^r\right)_{w, c} + \frac{d_c}{\vol(G)} \left(\bm{P}^r\right)_{c, w}
    \right).
    }Marginalizing $w$ and $c$ respectively reveals the fact that
    $
    \frac{\#(w)}{\abs{\mathcal{D} }} \overset{p}{\to} \frac{d_w}{\vol(G)}$
    and $
    \frac{\#(c)}{\abs{\mathcal{D} }} \overset{p}{\to} \frac{d_c}{\vol(G)}
    $, as $L\rightarrow\infty$.
\end{theorem}



\begin{restatable}{theorem}{dw}
\label{thm:dw} For DeepWalk,
%Let $A=D^{-1}W = I - L_{\text{rw}}$
when $L\rightarrow\infty$,
\beq{
\nonumber
\frac{\#(w, c) \abs{\mathcal{D} }}{\#(w) \cdot \#(c)} 
%\frac{m \sum_{r=1}^L \left( d_w M^r_{w, c} + d_c M^r_{c, w}\right)}{L d_w d_c} 
\overset{p}{\to} \frac{\vol(G)}{2T} \left( \frac{1}{d_c} \sum_{r=1}^T  \left(\bm{P}^r\right)_{w, c} +\frac{1}{d_w} \sum_{r=1}^T  \left(\bm{P}^r\right)_{c, w}\right).
}
\end{restatable}


$G=(V, E)$ to be an undirected, non-bipartite graph.
$(v_1, v_2, \cdots)$ is a stationary random walk.


==> overview.tex <==
\section{Overview}

In this document, we ...

==> simple.tex <==
\section{Simplified DeepWalk}

Let's have a simplified DeepWalk algorithm, as shown in Alg.~\ref{alg:dw_simple},
which only accounts for $T$-hop vertex pairs in multiset $\mathcal{D}$. 
The only difference is that we remove the inner loop at Line 5 of Alg.~\ref{alg:dw}.

\begin{algorithm}[h]
    \caption{Simplified DeepWalk}
    \label{alg:dw_simple}
    \For{$n = 1,2,\ldots, N$}{
    Sample a vertex $v^n_1$ from a distribution\;
    Generate a vertex sequence $(v^n_1, \cdots, v^n_L)$ of length $L$ by a random walk on graph $G$\;
    \For{$j = 1,2,\ldots, L-T$}{
        Add vertex-context pair $(v^n_j, v^n_{j+T})$ to multiset $\mathcal{D}$\;
        Add vertex-context pair $(v^n_{j+T}, v^n_j)$ to multiset $\mathcal{D}$\;
    }}
    Factorize a matrix with its entry at $w$-th row and $c$-th column to be $\log{\left(\frac{\#(w, c) \abs{\mathcal{D} }}{b\#(w) \cdot \#(c)}\right)}$.
    \end{algorithm}
    
    

\begin{definition}
 A Markov chain is ergodic if there is a number $N$ such that any state can be reached from any other state in any number of steps greater than or equal to a number $N$.
\end{definition}

\begin{theorem}
$X_i := (v_i, v_{i+1}, \cdots, v_{i+r})$ is an ergodic Markov Chain, with state space to be all $r$-step walks.
\end{theorem}
\begin{proof}
Want to show that $\exists M$, $\forall m>M$, $(v_0, \cdots, v_r)$ can reach $(u_0, \cdots, u_r)$.
We know $\{v_i\}_{i\geq 0}$ is ergodic, so there exists $N\geq r$ s.t., for any $n\geq N$, $v_r$ can reach $u_0$ at exact $n$ step.
Let the chain to be $(v_0, v_1, \cdots, v_r, \cdots, x_0, \cdots, x_{r-1}, u_0)$. The we construct a $n+r$ step walk 
from $(v_0, \cdots, v_r)$ to $(x_0, \cdots, x_{r-1}, u_0)$. Take further $r$ step,  we can reach $(u_0, \cdots, u_r)$,  
so we construct a $n+2r$ step walk from $(v_0, \cdots, v_r)$ to $(u_0, \cdots u_r)$. 
We then claim that any state can be reached from any other state in any number of 
steps greater than or equal to a number $N+2r$.
\end{proof}

The above theorem tells us $X_i = (v_i, \cdots, v_{i+r})$
is a ergodic markov chain on $V^{r+1}$ --- to be more rigorous, the space of all length-$r$ walks. 
 We define a matrix-value function:
\beq{
\besp{
    f: V^{r+1} &\longrightarrow \R^{d\times d}\\
     (v_i, \cdots, v_{i+r}) &\longmapsto \ve_{v_i} \otimes \ve_{v_{i+r}} + \ve_{v_{i+r}} \otimes \ve_{v_i} -  \frac{1}{\vol(G)} \mD\mP^r.
}}
In \cite{qiu2018network} we have proved that  
(1) under the stationary distribution, $\E[f(X)]=0$; 
and 
(2) $\frac{1}{k}\sum_{j=1}^k f(X_j) \overset{p}{\to} \vzero$.
We want to estimate the convergence rate.
